Tokenization Impacts Multilingual Language Modeling: Assessing Vocabulary Allocation and Overlap Across Languages

Multilingual language models have recently gained attention as a promising solution for representing multiple languages in a single model. In this paper, we propose new criteria to evaluate the quality of lexical representation and vocabulary overlap observed in sub-word tokenizers. Our findings show that the overlap of vocabulary across languages can be actually detrimental to certain downstream tasks (POS, dependency tree labeling). In contrast, NER and sentence-level tasks (cross-lingual retrieval, NLI) benefit from sharing vocabulary. We also observe that the coverage of the language-specific tokens in the multilingual vocabulary significantly impacts the word-level tasks. Our study offers a deeper understanding of the role of tokenizers in multilingual language models and guidelines for future model developers to choose the most suitable tokenizer for their specific application before undertaking costly model pre-training

==> figures/NER_F1_transfer.tex <==
\pdfoutput=1
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/NER_F1_transfer_.pdf}
    
    \caption{Cross-lingual transfer for Named Entity Recognition. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm. We observe a drop in cross-lingual transfer for \textsc{NoOverlap} tokenization, especially for the same script pairs, suggesting that lexical overlap is an important aspect contributing to cross-lingual transfer for NER.\jirka{maybe we should explain the colors in the heatmaps?}}
    \label{fig:ner_transfer}
\end{figure}

==> figures/NER_F1_transfer_20l.tex <==
\pdfoutput=1

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.\linewidth]{figures/NER_F1_transfer_20L.pdf}

    \caption{Cross-lingual transfer for Named Entity Recognition on 20 languages. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:ner_transfer_20l}
\end{figure*}

==> figures/POS_F1_transfer.tex <==
\pdfoutput=1

\begin{figure}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/POS_F1_transfer_.pdf}
    
    \caption{Cross-lingual transfer for Part of Speech Tagging The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:pos_transfer}
\end{figure}

==> figures/POS_F1_transfer_20l.tex <==
\pdfoutput=1
\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.\linewidth]{figures/POS_F1_transfer_20l_.pdf}

    \caption{Cross-lingual transfer for Part of Speech Tagging on 20 languages. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:pos_transfer_20l}
\end{figure*}

==> figures/Schwartz_figure.tex <==
\pdfoutput=1
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.9 \linewidth]{figures/Schwartz_figure.png}

    \caption{Mapping the impact of \va~and \vo~on language modelling. High \vo~benefits NER and sentence-level tasks (NLI, sentence retrieval) and hinders POS and dependency labeling performance. High \va~improves word-level tasks but leads to a decrease in masked language modeling scores. \tomasz{Make it look good}}
    \label{fig:schwartz}
\end{figure}

==> figures/Tatoeba_Acc_transfer.tex <==
\pdfoutput=1
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/Tatoeba_Acc_transfer_.pdf}
    
    \caption{Accuracy for cross-lingual sentence alignment, absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:tatoeba_transfer}
\end{figure}

==> figures/Tatoeba_Acc_transfer_20l.tex <==
\pdfoutput=1
\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.\linewidth]{figures/Tatoeba_Acc_transfer_20L.pdf}

    \caption{Accuracy for cross-lingual sentence alignment on 20 languages. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:tatoeba_transfer_20l}
\end{figure*}

==> figures/UD_F1_transfer.tex <==
\pdfoutput=1
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/UD_F1_transfer_.pdf}
    
    \caption{Cross-lingual transfer for dependency tree labeling. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:pos_transfer}
\end{figure}

==> figures/UD_F1_transfer_20l.tex <==
\pdfoutput=1
\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.\linewidth]{figures/UD_F1_transfer_20l_.pdf}

    \caption{Cross-lingual transfer for Dependency labeling on 20 languages. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:pos_transfer_20l}
\end{figure*}

==> figures/XNLI_Acc_transfer.tex <==
\pdfoutput=1
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/XNLI_Acc_transfer_.pdf}
    
    \caption{Cross-lingual transfer for Natural Language Inference, absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:xnli_transfer}
\end{figure}

==> figures/XNLI_Acc_transfer_20l.tex <==
\pdfoutput=1
\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.\linewidth]{figures/XNLI_Acc_transfer_20L.pdf}

    \caption{Cross-lingual transfer for Natural Language Inference, computed for 20 languages. The absolute values are presented for the Unigram tokenizer. For other tokenization methods, we show  the difference from the unigram algorithm.}
    \label{fig:xnli_transfer_20l}
\end{figure*}

==> figures/tokenizers_log_pdf_each_language.tex <==
\pdfoutput=1
\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/tokenizers_log_pdf_each_language_.pdf}
    
    \caption{Log-probabilites of vocabulary units in decreasing order for four tokenization methods. Results are divided by language.}
    \label{fig:tokenizers_log_pdf_each_language}
\end{figure*}

==> sections/X5_experiments.tex <==
\input{tables/in_lang_avg_combined.tex}
\input{figures/POS_NER_F1_merged.tex}

We train four tokenizers for the smaller set of diverse 6 languages (en, es, tr, el, zh, ar) using existing methods: Unigram, BPE, and our methods for monolingual tokenizer merging: \textsc{NoOverlap}, \textsc{TokMix}. Using these tokenizers, we then train four models\footnote{Details about the pretraining and probing procedures are described in Appendix~\ref{sec:model_architecture}} following the settings of XLM-Roberta \cite{conneau_unsupervised_2019} which we then use for the probing experiments. %The results reported for 6 language experiments are an average of 5 runs of probing with different seeds.

In Section~\ref{sec:tokenizer_results}, we analyze the distribution of learned vocabulary units and compute \va~and \vo~measures described in Section~\ref{sec:tokenization_measures}


Then in Section~\ref{sec:lm_results}, we evaluate the models' performance measures introduced in Section~\ref{sec:lm} and compare them with the measures for tokenizers.

Subsequently, we repeat the analysis for the broader set of 20 diverse languages (including six mentioned earlier and: he, ka, ur, hi, mr, th, ta, te, bg, ru, sw, vi, fr, de) with three tokenization methods used in three pre-trained models. In this setting, we do not use \textsc{NoOverlap} tokenizer, which cannot be trained effectively due to the necessity of constraining vocabulary for each language to $\frac{N}{L}=6,000$, which is too low for many of the analyzed languages. %We report an average of over 3 seeds for the 20 language experiments.


\subsection{Evaluation of Tokenizers' Properties}
\label{sec:tokenizer_results}

\jindrich{I like better when the paragraph headlines say the answers, not the questions.}

% \paragraph{What is the effective size of learned vocabularies?}

% \input{figures/tokenizers_log_pdf.tex}


% \tomasz{This may need to be moved to the appendix 93}
% In Figure~\ref{fig:tokenizers_log_pdf}, we present the probabilities of vocabulary units, computed on concatenate six languages corpora, learned by different tokenization algorithms. Unigram and \textsc{NoOVerlap} use a bigger fraction of the vocabulary for rarely appearing tokens (with probability lower than $10^{-6}$. BPE and \textsc{TokMix} produce a vast set of tokens with probabilities in the range between $10^{-5}$ and $10^{-6}$. Interestingly, the former algorithm allocates about 6000 vocabulary entries to tokens not appearing in the corpora. We further study the differences between learned vocabularies in Subsection~\ref{sec:learned_vocabularies}.


\paragraph{What portion of vocabulary is allocated to specific languages?}

%\input{figures/tokenizers_log_pdf_each_language.tex}
Table \ref{tab:vocab_allocation} shows that the average rank noticeably differs  across languages. The highest AR is observed for Chinese, which is caused by the fact that logographic scripts require an extensive vocabulary capacity to encode all characters. 

Multilingual vocabulary allocation is also highly dependent on the tokenization method used. Vocabulary learned  with Unigram has a comparable Average Rank with \textsc{NoOverlap}'s one, while the vocabularies of BPE and \textsc{TokMix} score higher in this metric. This observation holds throughout the languages, except for Chinese. Noticeably, \textsc{NoOverlap} vocabulary contains only 20,000 units for each of the languages, limiting the possible size of 
% and disallowing token overlap between them.

Moreover, Unigram tends to produce shorter tokens (measured by Characters per Token) than the other tokenization algorithms (again, except Chinese). 
%These observations suggest that vanilla Unigram is a suboptimal multilingual vocabulary learner. \tomasz{We present an in-depth analysis of the innate differences between presented tokenizers in the Appendix~\ref{sec:app_tokenizers}.}


\paragraph{Are similar lexical units used across languages?}

%\input{figures/jsd.tex}
Figure~\ref{fig:jsd_6l} shows Jensen-Shanon divergencies between the vocabularies of six languages. We observe that the highest cross-lingual overlaps appear in the vocabulary obtained by Unigram, followed by \textsc{TokMix}, and BPE. Expectedly, we do not observe overlaps for \textsc{NoOverlap}'s setting ($\mathrm{JSD}=1$).

Jensen-Shanon divergence is a good predictor of whether the languages share the script. For all tokenization methods, the divergence is significantly smaller in the bottom-right square grouping of the languages using Latin script. This effect is even more visible in the visualization of JSD computed for twenty languages (Figure~\ref{fig:jsd_20l} in Appendix~\ref{sec:app_results}).


\subsection{Tokenizer Properties Impact Language Model's Performance}
\label{sec:lm_results}

\input{tables/X_lang_combined.tex}

\paragraph{Is downstream performance affected by the tokenization method?}

% \input{tables/in_lang_keep.tex}


% Yes, for token-level tasks, F1 improves with lexical quality.

In Table~\ref{tab:in_lang_avg}, we observe that the change of the tokenization method leads to statistically significant changes in the F1 score for POS, dependency labeling, and NER. It may result from learning good lexical representations by BPE and \textsc{TokMix}, throughout languages, which is especially beneficial for word-level tasks. Whereas the influence on the sentence-level task (NLI) is minimal. The results confirm our assumption that \ va~ has a crucial effect on the quality of lexical information used in word-level tasks.
\jindrich{You should say if the significant differences are systematic or whether they seem random. Also, you should guide the reader on how to read the tables because there is too many numbers to quickly grasp what is going on.}


In contrast to the results of \cite{bostrom_byte_2020}, who found out that BPE underperforms Unigram on downstream tasks when used with a monolingual language model. We observe that in a multilingual setting, the former tokenization method learns better lexical representation throughout languages.


\paragraph{Does better performance on LM task translate to the improvement for downstream tasks?}

In Table~\ref{tab:in_lang_avg}, we observe that the models performing better on masked token prediction (MRR) tend to be worse on downstream tasks (POS and NER).\footnote{Noticeably, this trend does not hold for the averaged results for \textsc{NoOverlap} which search space in MLM task is constrained.}

We think that it's the result of different average rank. The higher it is, the more vocabulary units a language model needs to consider for masked token filling, making masked word prediction harder. At the same time, a high average rank means that language-specific vocabulary is broader and covers longer, thus more meaningful units. It leads to better results on downstream tasks within a language.


% In line with the observation of \cite{bostrom_byte_2020}, effective vocabulary allocation affects model performance. Unlike their observations for monolingual tokenization, we observe that in multilingual settings, sentence piece BPE tokenizer obtains better vocabulary allocation across languages that translate into an improvement on downstream tasks.

\paragraph{How does \vo~affect cross-lingual transfer?}


% \input{figures/NER_F1_transfer.tex}




We observed that \textsc{NoOverlap} approach obtains competitive results for POS tagging (highest average F1 in Table~\ref{tab:in_lang_avg}). Surprisingly no vocabulary sharing also improves cross-lingual transfer in the task among languages with Latin script (shown in Table~\ref{tab:X_lang} and Figure~\ref{fig:pos_transfer}). We think that the reason behind the strength of \textsc{NoOverlap} approach is that some tokens have different meanings across languages, e.g.,  the word ``a'' is an indefinite article in English and a preposition in Spanish.

Nevertheless, vocabulary overlap is crucial to cross-lingual transfer in some tasks.  Especially NER within the same script languages (Figure~\ref{fig:ner_transfer}) and sentence-level tasks. For these tasks, \textsc{NoOverlap} significantly underperforms other tokenization methods. The drop within Latin script languages: $6.8$ - $11.3\%$ for NER and $12.7$ - $15.9\%$ for sentence retrieval. In these cases, usage of the same tokens can indicate that texts refer to the same entities across languages, e.g., names are usually the same strings in the languages sharing writing system. 

Interestingly for word-level tasks, the best results are obtained from the approaches with the best in-lang scores even though they produce fewer shared tokens than Unigram. This observation hints that even for cross-lingual transfer, \va~is more important than \vo.

\paragraph{How do the results generalize to the larger set of languages?}

% \input{tables/in_lang_avg_20l.tex}
% \input{tables/X_lang_20L.tex}


We observe that the key observation for six language sets holds in the model trained for twenty languages. Table~\ref{tab:in_lang_avg_20l} shows that BPE and \textsc{TokMix} obtain better \va~than Unigram leading to improved results for word-level downstream tasks (NER, POS, Dependency labeling). Due to the lower vocab size to a number of languages ratio, average ranks decrease for all methods. as seen in Table~\ref{tab:in_lang_avg_20l}.

%\tomasz{Appendix candidate:}
Table~\ref{tab:X_lang_20L} shows that the cross-language vocabulary overlap is the highest for Unigram and lowest for BPE, similar yo the six languages settings. However, the association between \vo{} and the cross-lingual transfers is less pronounced. %\tomasz{I would get rid of 20 language Tatoeba results. They suffer from low bi-text coverage for 380 possible pairs, maybe just show en-xx accuracies ?}



\paragraph{Are proposed measures good predictors of the model's performance?}

\input{tables/corr_in_lang_20l_camread.tex}
\input{tables/corr_x_lang_20l_camread.tex}

In Table~\ref{tab:corr_in_lang_20l}, we show that the relationship between vocabulary quality (avg. rank and CPT) and LM performance (MRR) is statistically significant. The length of token units has a strong positive influence on POS, dependency labeling, and NER results ($r > 0.65$) and a negative influence on MRR ($r < 0.9$), while it does not significantly affect NLI results. The correlation between the average rank and MRR, NER scores is weaker but still significant. Moreover, it is significantly correlated with XNLI accuracy with a mediocre coefficient $r=0.56$, even though the changes in XNLI are low. 


\tomasz{Changed paragraph}
Table~\ref{tab:corr_x_lang_20l} presents the correlations for cross-lingual transfer scores with JSD measuring \vo. The coefficient supports our previous observation that lower overlap (thus higher JSD) improves transfer for POS tagging and dependency labeling and deteriorates it for other tasks. Although the correlation coefficients are significant, the association strength is weak, typically in the range: 0.1-0.2. It can be explained by the fact that the transfer is influenced by other factors, such as the in-language performance of the languages in the transfer pair. In the same table, we observe that the \va~s of source and target languages significantly influence the cross-lingual transfers for word-level tasks, with the higher impact of the target languages.

We describe the correlation analysis in detail in Appendix~\ref{sec:correlation_analysis}.


% \subsection{Learned Vocabularies Analysis}
% \label{sec:learned_vocabularies}
% \tomasz{Proabably to be moved to appendix 93}

% Why do different tokenization methods result in different allocations of vocabulary across languages?


% \paragraph{Why BPE is better than Unigram in vocabulary allocation throughout languages?}

% \input{figures/AR_x_vocabulary.tex}
% \input{figures/CPT_x_vocabulary.tex}

% To answer this question, we train Unigram and BPE tokenizers for different vocabulary sizes. We observe that both the average rank (Figure~\ref{fig:ar_vocab}) and CPT (Figure~\ref{fig:cpt_vocab}) stop rising for vocab sizes above 250,000 (with the exception of Chinese). For BPE, the metrics still steadily rise after this threshold, which makes it overperform Unigram for most languages.

% We think that the reason why Unigram does not learn useful tokens after this point is the way the initial vocabulary is constructed, i.e., it is the set of all character n-grams appearing in the corpus with n lower than 16. In contrast to BPR, Unigram's vocabulary won't cover longer words than 16 characters, which can be useful in some languages.

% We think that further work on identifying optimal strategies for tokenization is still needed in the future. 

% \paragraph{Which units are preferred by specific tokenizers?}
% \input{tables/learned_vocab_comparison.tex}

% In Table~\ref{tab:learned_vocab_comparison}, we show the tokens with the highest differences in empirical probabilities obtained with BPE and Unigram tokenizers for three languages. We see that Unigram prefers suffixes to prefixes of words. Also, it splits text more often into single, which may be due to lower average rank for specific languages.


==> tables/X_lang.tex <==
\begin{table}

\centering
\caption{Results of evaluation for cros-languages overlaps and transfers for six diverse languages.We observe significant changes for different tokenization methods.}
\label{tab:X_lang}
\small
\begin{tabular}{lllll}
\toprule
        &        &       diff-script &       same-script &               all \\
metric & tokenizer &                   &                   &                   \\
\midrule
\multirow{4}{*}{JSD} & Unigram &              0.77 &              0.62 &              0.74 \\
        & BPE &              0.83 &              0.68 &               0.8 \\
        & NoOverlap &               1.0 &               1.0 &               1.0 \\
        & TokMix &               0.8 &              0.65 &              0.77 \\
\cline{1-5}
\multirow{4}{*}{NER} & Unigram &  31.3 $_{\pm0.4}$ &  55.4 $_{\pm0.2}$ &  36.1 $_{\pm0.4}$ \\
        & BPE &  33.5 $_{\pm0.5}$ &  59.9 $_{\pm0.2}$ &  38.7 $_{\pm0.4}$ \\
        & NoOverlap &  32.0 $_{\pm0.5}$ &  48.6 $_{\pm0.4}$ &  35.3 $_{\pm0.5}$ \\
        & TokMix &  31.8 $_{\pm0.4}$ &  58.0 $_{\pm0.3}$ &  37.0 $_{\pm0.4}$ \\
\cline{1-5}
\multirow{4}{*}{POS} & Unigram &  18.1 $_{\pm0.4}$ &  38.3 $_{\pm0.4}$ &  22.2 $_{\pm0.4}$ \\
        & BPE &  25.8 $_{\pm0.5}$ &  40.8 $_{\pm0.4}$ &  28.8 $_{\pm0.5}$ \\
        & NoOverlap &  20.1 $_{\pm0.5}$ &  41.9 $_{\pm0.5}$ &  24.5 $_{\pm0.5}$ \\
        & TokMix &  21.9 $_{\pm0.4}$ &  40.4 $_{\pm0.3}$ &  25.6 $_{\pm0.4}$ \\
\cline{1-5}
\multirow{4}{*}{UD} & Unigram &  11.1 $_{\pm0.3}$ &  25.5 $_{\pm0.3}$ &  14.0 $_{\pm0.3}$ \\
        & BPE &  15.9 $_{\pm0.4}$ &  27.0 $_{\pm0.4}$ &  18.1 $_{\pm0.4}$ \\
        & NoOverlap &  12.8 $_{\pm0.4}$ &  27.8 $_{\pm0.5}$ &  15.8 $_{\pm0.4}$ \\
        & TokMix &  12.6 $_{\pm0.5}$ &  26.1 $_{\pm0.3}$ &  15.3 $_{\pm0.5}$ \\
\cline{1-5}
\multirow{4}{*}{XNLI} & Unigram &  42.2 $_{\pm0.7}$ &  43.7 $_{\pm0.7}$ &  42.5 $_{\pm0.7}$ \\
        & BPE &  42.4 $_{\pm0.7}$ &  45.2 $_{\pm0.8}$ &  43.0 $_{\pm0.7}$ \\
        & NoOverlap &  37.3 $_{\pm0.6}$ &  37.1 $_{\pm0.5}$ &  37.2 $_{\pm0.6}$ \\
        & TokMix &  41.2 $_{\pm0.7}$ &  42.7 $_{\pm0.5}$ &  41.5 $_{\pm0.7}$ \\
\cline{1-5}
\multirow{4}{*}{Tatoeba} & Unigram &              21.0 &              43.9 &              25.6 \\
        & BPE &              20.9 &              40.7 &              24.9 \\
        & NoOverlap &              12.3 &              28.0 &              15.4 \\
        & TokMix &              23.0 &              43.4 &              27.1 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/X_lang_20L.tex <==
\begin{table}
\centering
\caption{Results of evaluation for cros-languages overlaps and transfers for twenty diverse languages.We observe significant changes for different tokenization methods.}
\label{tab:X_lang_20L}
\small
\begin{tabular}{lllll}
\toprule
        &        &       diff-script &       same-script &               all \\
metric & tokenizer &                   &                   &                   \\
\midrule
\multirow{3}{*}{JSD} & Unigram &              0.75 &              0.58 &              0.73 \\
        & BPE &              0.83 &              0.67 &              0.81 \\
        & TokMix &               0.8 &              0.64 &              0.78 \\
\cline{1-5}
\multirow{3}{*}{NER} & Unigram &  33.2 $_{\pm0.5}$ &  50.7 $_{\pm0.6}$ &  35.4 $_{\pm0.5}$ \\
        & BPE &  36.6 $_{\pm0.6}$ &  54.3 $_{\pm0.3}$ &  38.8 $_{\pm0.5}$ \\
        & TokMix &  36.5 $_{\pm0.6}$ &  53.7 $_{\pm0.5}$ &  38.7 $_{\pm0.6}$ \\
\cline{1-5}
\multirow{3}{*}{POS} & Unigram &  23.4 $_{\pm0.5}$ &  32.9 $_{\pm0.3}$ &  24.6 $_{\pm0.5}$ \\
        & BPE &  30.5 $_{\pm0.6}$ &  40.7 $_{\pm0.4}$ &  31.8 $_{\pm0.6}$ \\
        & TokMix &  29.2 $_{\pm0.5}$ &  40.4 $_{\pm0.3}$ &  30.7 $_{\pm0.5}$ \\
\cline{1-5}
\multirow{3}{*}{UD} & Unigram &  13.0 $_{\pm0.6}$ &  15.6 $_{\pm0.5}$ &  13.4 $_{\pm0.6}$ \\
        & BPE &  16.5 $_{\pm0.6}$ &  19.2 $_{\pm0.5}$ &  16.9 $_{\pm0.5}$ \\
        & TokMix &  16.0 $_{\pm0.5}$ &  19.4 $_{\pm0.4}$ &  16.5 $_{\pm0.5}$ \\
\cline{1-5}
\multirow{3}{*}{XNLI} & Unigram &  37.3 $_{\pm0.5}$ &  37.5 $_{\pm0.4}$ &  37.4 $_{\pm0.5}$ \\
        & BPE &  36.2 $_{\pm0.5}$ &  38.7 $_{\pm0.5}$ &  36.7 $_{\pm0.5}$ \\
        & TokMix &  37.8 $_{\pm0.5}$ &  39.2 $_{\pm0.5}$ &  38.1 $_{\pm0.5}$ \\
\cline{1-5}
\multirow{3}{*}{Tatoeba} & Unigram &              44.1 &              44.4 &              44.2 \\
        & BPE &              44.1 &              49.1 &              45.1 \\
        & TokMix &              42.8 &              46.9 &              43.6 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/corr_in_lang.tex <==
\begin{table}
\centering
\caption{Correlations between task performance metrics and tokenizer measures.Stars denote statistical significance: (* coresponeds to $p<0.05$ and ** to $p<0.01$).}
\label{tab:corr_in_lang}
\begin{tabular}{llll}
\toprule
metric & Avg. Rank &       CPT &       MRR \\
metric &           &           &           \\
\midrule
CPT    &   0.863** &       1.0 &  -0.861** \\
MRR    &  -0.836** &  -0.861** &       1.0 \\
NER    &     0.332 &    0.478* &    -0.326 \\
POS    &     0.123 &     0.403 &    -0.215 \\
UD     &     0.049 &     0.286 &    -0.129 \\
XNLI   &     0.269 &      0.07 &    -0.013 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/corr_in_lang_20l.tex <==
\begin{table}
\centering
\caption{Correlations between task performance metrics and tokenizer measures.Stars denote statistical significance: (* coresponeds to $p<0.05$ and ** to $p<0.01$).}
\label{tab:corr_in_lang_20l}
\begin{tabular}{llll}
\toprule
metric & Avg. Rank &       CPT &       MRR \\
metric &           &           &           \\
\midrule
CPT    &    0.79** &       1.0 &  -0.913** \\
MRR    &  -0.723** &  -0.913** &       1.0 \\
NER    &   0.394** &   0.657** &  -0.745** \\
POS    &     0.32* &   0.724** &  -0.754** \\
UD     &     0.266 &   0.675** &  -0.695** \\
XNLI   &    0.56** &    0.388* &  -0.437** \\
\bottomrule
\end{tabular}
\end{table}


==> tables/corr_in_lang_20l_keep.tex <==
\begin{table}
\footnotesize
\centering

\begin{tabular}{lccc|c}
\toprule
 & \multicolumn{2}{c}{\bf{V. Allocation}} & \bf{MLM} & \bf{V. Overlap} \\
 & (AR) &  (CPT)  &  (MRR) & (JSD) \\
\midrule
CPT    &    \bf{0.790} &     - &  - & - \\
MRR    &  \bf{-0.723} &  \bf{-0.913} &  - & - \\
NER    &   \bf{0.394} &   \bf{0.657} &  \bf{-0.745} & \bf{-0.153}\\
POS    &     0.320 &   \bf{0.724} &  \bf{-0.754} & \bf{0.164}  \\
Dep l. &     0.266 &   \bf{0.675} &  \bf{-0.695} & \bf{0.095} \ \\
NLI   &    \bf{0.56} &    0.388 &  \bf{-0.437} & \bf{-0.236} \\
Retrieval & - & - & - & \bf{-0.157} \\ 
\bottomrule
\end{tabular}
\caption{Spearman correlations between task coefficients performance metrics and tokenizer measures. The first three columns (\va~and MLM) correspond to the in-language results. The last column presents correlations between \vo~ measure (``JSD'') and cross-lingual transfer results. Statistically significant correlations ($p<0.01$) are bolded. \tomasz{Add separate table with the results for cross-lingual transfer.}}
\label{tab:corr_in_lang_20l}
\end{table}


==> tables/corr_x_lang_20l_camread.tex <==
\begin{table*}
\centering
\begin{tabular}{lcccccc}
\toprule
 & \bf{V. Overlap} & \multicolumn{2}{c}{\bf{V. Allocation SRC}}  & \multicolumn{2}{c}{\bf{V. Allocation TGT}} \\ 
 & (JSD) &  (AR)  &  (CPT) & (AR) & (CPT) \\ \midrule
% NER     &  \bf{-0.153} &        0.061 &  \bf{0.174} &   \bf{0.180} &   \bf{0.250} \\
% POS     &   \bf{0.164} &       \bf{0.187} &  \bf{0.366} &       \bf{0.238} &  \bf{0.379} \\
% Dep l.     &   \bf{0.095} &      \bf{ 0.095} &  \bf{0.216} &       \bf{0.134} &  \bf{0.232} \\
% NLI    &  \bf{-0.234} &         -0.060 &   -0.025 &       -0.079 &   -0.071 \\
% Retrieval &  \bf{-0.157} &         0.041 &    0.023 &         0.031 &     0.020 \\
NER     &  \bf{0.553} &       \bf{0.172} &  \bf{0.412} &      \bf{0.409} &  \bf{0.568} \\
POS     &  \bf{0.759} &       \bf{0.383} &   \bf{0.69} &       \bf{0.436} &  \bf{0.714} \\
Dep l.     &  \bf{0.596} &       \bf{0.314} &  \bf{0.587} &       \bf{0.351} &  \bf{0.605} \\
NLI    &  -0.078 &        -0.039 &   -0.006 &       -0.083 &  -0.082 \\
Retrieval &  \bf{0.156} &       \bf{0.214} &  \bf{0.139} &       \bf{0.214} &  \bf{0.144} \\
\bottomrule
\end{tabular}
\caption{Spearman correlations between cross-lingual transfer results and tokenization measures. \vo~is measured by JSD, we also measure the correlation with \va s of source and target language of the transfer directions. Statistically significant correlations ($p<0.01$) are bolded. Computed for 20 languages.}
\label{tab:corr_x_lang_20l}
\end{table*}


==> tables/in_lang.tex <==
\begin{table}
\centering
\begin{tabular}{lllllllll}
\toprule
     &        &                ar &                tr &                zh &                el &                es &                en &               All \\
metric & tokenizer &                   &                   &                   &                   &                   &                   &                   \\
\midrule
\multirow{4}{*}{Avg. Rank} & Unigram &              2129 &              2719 &              5919 &              2070 &              1439 &              1513 &              2042 \\
     & BPE &              2972 &              3226 &              4294 &              2907 &              2220 &              2143 &              2193 \\
     & NoOverlap &              2537 &              2653 &              2090 &              2065 &              1661 &              1597 &              1829 \\
     & TokMix &              3485 &              4167 &              3961 &              2639 &              1999 &              1898 &              2198 \\
\cline{1-9}
\multirow{4}{*}{CPT} & Unigram &              3.16 &              4.01 &              1.84 &               3.5 &              3.88 &              3.91 &              3.17 \\
     & BPE &               3.7 &              4.19 &              2.03 &              3.97 &              4.34 &              4.22 &              4.47 \\
     & NoOverlap &              3.53 &              4.19 &              1.56 &              3.81 &              4.15 &              4.15 &              3.16 \\
     & TokMix &               3.7 &              4.45 &              1.73 &               3.9 &              4.24 &              4.18 &              3.34 \\
\cline{1-9}
\multirow{4}{*}{MRR} & Unigram &              36.0 &              36.0 &              34.2 &              46.3 &              49.7 &              49.6 &              42.0 \\
     & BPE &              28.7 &              33.6 &              28.6 &              38.6 &              43.1 &              41.0 &              35.6 \\
     & NoOverlap &              38.1 &              39.6 &              41.4 &              42.8 &              47.5 &              46.6 &              42.7 \\
     & TokMix &              31.5 &              30.6 &              38.2 &              41.2 &              45.3 &              45.6 &              38.7 \\
\cline{1-9}
\multirow{4}{*}{NER} & Unigram &  66.4 $_{\pm0.1}$ &  73.0 $_{\pm0.1}$ &  35.1 $_{\pm0.1}$ &  68.0 $_{\pm0.1}$ &  68.0 $_{\pm0.1}$ &  66.1 $_{\pm0.2}$ &  62.8 $_{\pm0.1}$ \\
     & BPE &  76.1 $_{\pm0.0}$ &  76.7 $_{\pm0.0}$ &  54.2 $_{\pm0.1}$ &  70.3 $_{\pm0.1}$ &  75.2 $_{\pm0.1}$ &  70.0 $_{\pm0.0}$ &  70.4 $_{\pm0.1}$ \\
     & NoOverlap &  76.5 $_{\pm0.1}$ &  72.8 $_{\pm0.0}$ &  58.4 $_{\pm0.1}$ &  69.6 $_{\pm0.1}$ &  71.6 $_{\pm0.1}$ &  67.3 $_{\pm0.1}$ &  69.4 $_{\pm0.1}$ \\
     & TokMix &  76.6 $_{\pm0.1}$ &  76.2 $_{\pm0.1}$ &  56.1 $_{\pm0.0}$ &  70.1 $_{\pm0.1}$ &  74.3 $_{\pm0.1}$ &  68.1 $_{\pm0.1}$ &  70.2 $_{\pm0.1}$ \\
\cline{1-9}
\multirow{4}{*}{POS} & Unigram &  54.8 $_{\pm0.1}$ &  46.9 $_{\pm0.2}$ &  29.3 $_{\pm0.1}$ &  52.9 $_{\pm0.3}$ &  76.5 $_{\pm0.2}$ &  81.9 $_{\pm0.1}$ &  57.1 $_{\pm0.2}$ \\
     & BPE &  66.7 $_{\pm0.1}$ &  52.1 $_{\pm0.1}$ &  62.2 $_{\pm0.0}$ &  63.4 $_{\pm0.1}$ &  81.7 $_{\pm0.4}$ &  87.4 $_{\pm0.1}$ &  68.9 $_{\pm0.2}$ \\
     & NoOverlap &  66.5 $_{\pm0.1}$ &  52.5 $_{\pm0.2}$ &  60.6 $_{\pm0.1}$ &  67.5 $_{\pm0.1}$ &  81.3 $_{\pm0.6}$ &  86.7 $_{\pm0.1}$ &  69.2 $_{\pm0.2}$ \\
     & TokMix &  66.0 $_{\pm0.1}$ &  52.1 $_{\pm0.2}$ &  56.2 $_{\pm0.0}$ &  61.7 $_{\pm0.2}$ &  81.3 $_{\pm0.2}$ &  86.3 $_{\pm0.1}$ &  67.3 $_{\pm0.1}$ \\
\cline{1-9}
\multirow{4}{*}{UD} & Unigram &  13.5 $_{\pm0.6}$ &  58.6 $_{\pm0.8}$ &  20.7 $_{\pm0.1}$ &  58.4 $_{\pm0.4}$ &  71.9 $_{\pm0.1}$ &  65.7 $_{\pm0.2}$ &  48.1 $_{\pm0.4}$ \\
     & BPE &  13.8 $_{\pm0.0}$ &  63.7 $_{\pm1.2}$ &  59.5 $_{\pm0.1}$ &  68.2 $_{\pm0.8}$ &  77.0 $_{\pm0.2}$ &  70.3 $_{\pm0.4}$ &  58.7 $_{\pm0.4}$ \\
     & NoOverlap &  13.2 $_{\pm0.0}$ &  65.0 $_{\pm0.5}$ &  60.5 $_{\pm0.2}$ &  67.7 $_{\pm0.2}$ &  77.1 $_{\pm0.3}$ &  69.2 $_{\pm0.3}$ &  58.8 $_{\pm0.3}$ \\
     & TokMix &  14.1 $_{\pm0.0}$ &  62.9 $_{\pm1.2}$ &  53.8 $_{\pm0.1}$ &  67.3 $_{\pm0.5}$ &  76.5 $_{\pm0.1}$ &  69.1 $_{\pm0.2}$ &  57.3 $_{\pm0.4}$ \\
\cline{1-9}
\multirow{4}{*}{XNLI} & Unigram &  52.5 $_{\pm0.3}$ &  52.9 $_{\pm0.3}$ &  47.5 $_{\pm1.4}$ &  55.0 $_{\pm0.2}$ &  55.3 $_{\pm0.3}$ &  57.4 $_{\pm0.5}$ &  53.4 $_{\pm0.5}$ \\
     & BPE &  52.2 $_{\pm0.3}$ &  53.6 $_{\pm0.5}$ &  45.2 $_{\pm0.4}$ &  55.6 $_{\pm0.3}$ &  55.7 $_{\pm0.2}$ &  57.8 $_{\pm0.2}$ &  53.3 $_{\pm0.3}$ \\
     & NoOverlap &  52.9 $_{\pm0.7}$ &  54.0 $_{\pm0.2}$ &  44.0 $_{\pm0.8}$ &  54.8 $_{\pm0.1}$ &  54.9 $_{\pm0.3}$ &  57.3 $_{\pm0.3}$ &  53.0 $_{\pm0.4}$ \\
     & TokMix &  52.0 $_{\pm0.2}$ &  53.6 $_{\pm0.5}$ &  46.2 $_{\pm1.0}$ &  55.4 $_{\pm0.3}$ &  55.3 $_{\pm0.1}$ &  57.5 $_{\pm0.2}$ &  53.3 $_{\pm0.4}$ \\
\bottomrule
\end{tabular}
\caption{Results of evaluation for in-language properties and tasks for six diverse languages. We observe significant changes for different tokenization methods. The results for MRR, POS, NER, XNLI are in percent. For the downstream task, we show average and standard deviations computed for five runs of probing.}
\label{tab:in_lang}
\end{table}


==> tables/in_lang_avg.tex <==
\begin{table}
\centering
\caption{Results of evaluation for in language properties and tasks averaged six diverse languages.We observe significant changes for different tokenization methods.}
\label{tab:in_lang_avg}
\small
\begin{tabular}{llllllll}
\toprule
metric & Avg. Rank &   CPT &   MRR &               NER &               POS &                UD &              XNLI \\
tokenizer &           &       &       &                   &                   &                   &                   \\
\midrule
Unigram   &      2042 &  3.17 &  42.0 &  62.8 $_{\pm0.1}$ &  57.1 $_{\pm0.2}$ &  48.1 $_{\pm0.4}$ &  53.4 $_{\pm0.5}$ \\
BPE       &      2193 &  4.47 &  35.6 &  70.4 $_{\pm0.1}$ &  68.9 $_{\pm0.2}$ &  58.7 $_{\pm0.4}$ &  53.3 $_{\pm0.3}$ \\
NoOverlap &      1829 &  3.16 &  42.7 &  69.4 $_{\pm0.1}$ &  69.2 $_{\pm0.2}$ &  58.8 $_{\pm0.3}$ &  53.0 $_{\pm0.4}$ \\
TokMix    &      2198 &  3.34 &  38.7 &  70.2 $_{\pm0.1}$ &  67.3 $_{\pm0.1}$ &  57.3 $_{\pm0.4}$ &  53.3 $_{\pm0.4}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/in_lang_avg_20l.tex <==
\begin{table}
\centering
\caption{Results of evaluation for in language properties and tasks for twenty diverse languages.We observe significant changes for different tokenization methods.}
\label{tab:in_lang_avg_20l}
    \small
    \begin{tabular}{llllllll}
    \toprule
    metric & Avg. Rank &   CPT &   MRR &               NER &               POS &                UD &              XNLI \\
    tokenizer &           &       &       &                   &                   &                   &                   \\
    \midrule
    Unigram   &       623 &  2.89 &  52.6 &  58.9 $_{\pm0.2}$ &  54.0 $_{\pm0.4}$ &  43.7 $_{\pm0.4}$ &  53.2 $_{\pm0.3}$ \\
    BPE       &       809 &  3.43 &  40.5 &  66.3 $_{\pm0.2}$ &  67.3 $_{\pm0.4}$ &  54.5 $_{\pm0.5}$ &  53.5 $_{\pm0.3}$ \\
    TokMix    &       689 &  3.23 &  44.8 &  65.4 $_{\pm0.3}$ &  66.5 $_{\pm0.4}$ &  53.9 $_{\pm0.5}$ &  52.3 $_{\pm0.3}$ \\
    \bottomrule
    \end{tabular}
    \end{table}
    

==> tables/in_lang_table_20l.tex <==
\begin{landscape}
\begin{table}
\centering
\small
\scalebox{0.6}{
\begin{tabular}{lllllllllllllllllllllll}
\toprule
     &        &                ar &                tr &                zh &                el &                es &                en &                sw &                hi &                mr &                ur &                ta &                te &                th &                ru &                bg &                he &                ka &                vi &                fr &                de &               All \\
metric & tokenizer &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   \\
\midrule
\multirowcell{4}[0pt][l]{\textbf{V. Allocation} \\ (AR)} & Unigram &               998 &              1542 &              3033 &              1023 &               866 &              1006 &               688 &               691 &               821 &               431 &               991 &               832 &              1680 &              1308 &              1284 &               978 &              1008 &               232 &               860 &              1087 &               623 \\
     & BPE &              1378 &              1737 &              1435 &              1322 &              1374 &              1508 &              1067 &              1150 &              1128 &               758 &               974 &               932 &              1826 &              1953 &              1566 &              1317 &              1103 &               859 &              1377 &              1531 &               809 \\
     & TokMix &              1141 &              1805 &              1632 &               849 &              1031 &              1178 &              1263 &              1153 &              1471 &               771 &              1323 &              1307 &              1477 &              1137 &              1078 &              1117 &              1178 &               748 &              1019 &              1130 &               689 \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{V. Allocation} \\ (CPT)} & Unigram &              2.71 &              3.45 &              1.65 &              2.93 &              3.31 &              3.43 &              3.11 &               2.7 &              2.86 &              2.61 &              3.42 &              2.97 &              3.45 &              3.31 &              3.14 &               2.5 &               3.1 &              2.24 &              3.24 &              3.51 &              2.89 \\
     & BPE &              3.22 &              3.65 &              2.05 &              3.44 &              3.96 &              3.98 &              3.76 &              3.33 &              3.31 &              3.39 &               3.5 &              3.19 &              3.53 &              3.81 &              3.49 &               3.0 &              3.33 &              3.62 &              3.92 &              3.95 &              3.43 \\
     & TokMix &              3.06 &              3.79 &              1.52 &              3.13 &              3.73 &              3.84 &              4.15 &              3.37 &              3.56 &              3.42 &              3.79 &              3.52 &              3.36 &              3.38 &               3.2 &              2.86 &              3.38 &              3.49 &              3.69 &              3.82 &              3.23 \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{MLM} \\ (MRR)} & Unigram &              48.0 &              44.3 &              42.9 &              58.1 &              57.0 &              54.7 &              60.0 &              57.8 &              50.9 &              58.9 &              43.4 &              52.5 &              41.0 &              53.9 &              50.6 &              54.6 &              49.7 &              62.6 &              57.3 &              54.1 &              52.6 \\
     & BPE &              34.1 &              36.1 &              29.8 &              48.2 &              44.3 &              41.7 &              46.9 &              42.8 &              39.8 &              42.9 &              35.3 &              42.2 &              34.5 &              43.5 &              41.4 &              34.2 &              41.4 &              43.8 &              44.3 &              43.3 &              40.5 \\
     & TokMix &              38.2 &              39.1 &              43.2 &              53.5 &              48.5 &              48.1 &              43.0 &              44.8 &              39.8 &              44.0 &              38.2 &              43.8 &              40.8 &              51.2 &              47.4 &              43.2 &              44.2 &              47.2 &              49.7 &              47.8 &              44.8 \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{NER} \\ (F1)} & Unigram &  60.4 $_{\pm0.1}$ &  73.0 $_{\pm0.1}$ &  32.4 $_{\pm0.1}$ &  67.3 $_{\pm0.1}$ &  71.1 $_{\pm0.0}$ &  65.9 $_{\pm0.1}$ &  41.1 $_{\pm0.2}$ &  57.1 $_{\pm0.3}$ &  61.3 $_{\pm0.6}$ &  71.8 $_{\pm0.1}$ &  61.1 $_{\pm0.3}$ &  13.2 $_{\pm0.9}$ &  34.3 $_{\pm0.1}$ &  70.2 $_{\pm0.1}$ &  72.9 $_{\pm0.1}$ &  54.5 $_{\pm0.1}$ &  58.1 $_{\pm0.1}$ &  74.0 $_{\pm0.1}$ &  71.3 $_{\pm0.0}$ &  66.5 $_{\pm0.0}$ &  58.9 $_{\pm0.2}$ \\
     & BPE &  76.0 $_{\pm0.1}$ &  77.6 $_{\pm0.1}$ &  54.5 $_{\pm0.1}$ &  70.5 $_{\pm0.1}$ &  74.6 $_{\pm0.0}$ &  70.4 $_{\pm0.1}$ &  54.3 $_{\pm1.2}$ &  65.7 $_{\pm0.3}$ &  66.4 $_{\pm0.1}$ &  82.5 $_{\pm0.1}$ &  66.6 $_{\pm0.3}$ &  15.0 $_{\pm1.5}$ &  43.3 $_{\pm0.0}$ &  72.6 $_{\pm0.0}$ &  75.9 $_{\pm0.1}$ &  64.4 $_{\pm0.1}$ &  72.3 $_{\pm0.2}$ &  78.6 $_{\pm0.0}$ &  74.4 $_{\pm0.0}$ &  70.6 $_{\pm0.0}$ &  66.3 $_{\pm0.2}$ \\
     & TokMix &  75.9 $_{\pm0.1}$ &  75.4 $_{\pm0.0}$ &  56.2 $_{\pm0.1}$ &  68.9 $_{\pm0.1}$ &  73.6 $_{\pm0.1}$ &  69.3 $_{\pm0.0}$ &  48.8 $_{\pm3.1}$ &  65.1 $_{\pm0.3}$ &  66.1 $_{\pm0.2}$ &  82.5 $_{\pm0.1}$ &  66.0 $_{\pm0.3}$ &  15.1 $_{\pm0.8}$ &  41.3 $_{\pm0.0}$ &  71.4 $_{\pm0.1}$ &  75.2 $_{\pm0.1}$ &  64.4 $_{\pm0.2}$ &  70.5 $_{\pm0.0}$ &  78.5 $_{\pm0.1}$ &  73.7 $_{\pm0.1}$ &  69.5 $_{\pm0.1}$ &  65.4 $_{\pm0.3}$ \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{POS} \\ (F1)} & Unigram &  50.0 $_{\pm0.1}$ &  43.4 $_{\pm0.2}$ &  21.6 $_{\pm0.0}$ &  43.6 $_{\pm0.2}$ &  72.4 $_{\pm0.2}$ &  76.7 $_{\pm0.1}$ &                 - &  66.9 $_{\pm0.1}$ &  20.5 $_{\pm2.9}$ &  65.5 $_{\pm0.1}$ &  23.0 $_{\pm1.4}$ &  30.5 $_{\pm0.8}$ &                 - &  74.8 $_{\pm0.0}$ &  77.9 $_{\pm0.3}$ &  67.9 $_{\pm0.1}$ &                 - &  40.0 $_{\pm0.5}$ &  72.7 $_{\pm0.1}$ &  70.7 $_{\pm0.0}$ &  54.0 $_{\pm0.4}$ \\
     & BPE &  66.2 $_{\pm0.0}$ &  51.7 $_{\pm0.1}$ &  59.2 $_{\pm0.1}$ &  64.8 $_{\pm0.1}$ &  82.2 $_{\pm0.1}$ &  87.4 $_{\pm0.1}$ &                 - &  74.6 $_{\pm0.0}$ &  27.9 $_{\pm1.5}$ &  83.6 $_{\pm0.4}$ &  25.2 $_{\pm0.6}$ &  33.9 $_{\pm2.0}$ &                 - &  84.6 $_{\pm0.1}$ &  88.6 $_{\pm0.3}$ &  82.7 $_{\pm0.0}$ &                 - &  66.2 $_{\pm0.4}$ &  83.4 $_{\pm0.1}$ &  82.5 $_{\pm0.0}$ &  67.3 $_{\pm0.4}$ \\
     & TokMix &  65.9 $_{\pm0.1}$ &  51.2 $_{\pm0.1}$ &  55.3 $_{\pm0.1}$ &  60.7 $_{\pm0.1}$ &  81.7 $_{\pm0.2}$ &  86.6 $_{\pm0.1}$ &                 - &  74.9 $_{\pm0.0}$ &  25.6 $_{\pm1.3}$ &  82.6 $_{\pm0.2}$ &  28.6 $_{\pm2.3}$ &  32.5 $_{\pm0.9}$ &                 - &  84.6 $_{\pm0.0}$ &  87.9 $_{\pm0.1}$ &  83.3 $_{\pm0.2}$ &                 - &  64.9 $_{\pm0.3}$ &  81.4 $_{\pm0.1}$ &  82.7 $_{\pm0.8}$ &  66.5 $_{\pm0.4}$ \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{Dep. labeling} \\ (F1)} & Unigram &  12.0 $_{\pm0.0}$ &  56.9 $_{\pm0.2}$ &  15.3 $_{\pm0.1}$ &  52.4 $_{\pm0.1}$ &  67.3 $_{\pm0.1}$ &  61.6 $_{\pm0.1}$ &                 - &  78.4 $_{\pm0.2}$ &  22.0 $_{\pm1.2}$ &  59.0 $_{\pm0.4}$ &  33.5 $_{\pm0.3}$ &  29.2 $_{\pm1.5}$ &                 - &  44.1 $_{\pm0.4}$ &  64.9 $_{\pm1.3}$ &  49.6 $_{\pm0.3}$ &                 - &  35.6 $_{\pm0.2}$ &  12.8 $_{\pm0.0}$ &  48.6 $_{\pm0.3}$ &  43.7 $_{\pm0.4}$ \\
     & BPE &  13.3 $_{\pm0.5}$ &  62.7 $_{\pm1.2}$ &  56.1 $_{\pm0.2}$ &  67.7 $_{\pm0.4}$ &  77.1 $_{\pm0.4}$ &  70.2 $_{\pm0.3}$ &                 - &  85.7 $_{\pm0.0}$ &  24.6 $_{\pm1.4}$ &  74.6 $_{\pm0.1}$ &  40.2 $_{\pm1.0}$ &  36.0 $_{\pm1.7}$ &                 - &  55.1 $_{\pm0.2}$ &  76.3 $_{\pm0.1}$ &  63.2 $_{\pm0.0}$ &                 - &  49.9 $_{\pm0.2}$ &  12.4 $_{\pm0.0}$ &  61.5 $_{\pm0.3}$ &  54.5 $_{\pm0.5}$ \\
     & TokMix &  10.0 $_{\pm0.0}$ &  64.6 $_{\pm1.0}$ &  54.0 $_{\pm0.1}$ &  67.5 $_{\pm0.5}$ &  76.9 $_{\pm0.2}$ &  69.0 $_{\pm0.1}$ &                 - &  86.2 $_{\pm0.1}$ &  24.9 $_{\pm1.2}$ &  75.3 $_{\pm0.5}$ &  39.6 $_{\pm0.9}$ &  34.7 $_{\pm0.9}$ &                 - &  54.0 $_{\pm0.5}$ &  74.2 $_{\pm0.8}$ &  63.0 $_{\pm1.0}$ &                 - &  49.4 $_{\pm0.4}$ &  11.2 $_{\pm0.0}$ &  61.5 $_{\pm0.0}$ &  53.9 $_{\pm0.5}$ \\
\cline{1-23}
\multirowcell{4}[0pt][l]{\textbf{NLI} \\ (Acc)} & Unigram &  51.6 $_{\pm0.3}$ &  53.4 $_{\pm0.2}$ &  48.4 $_{\pm0.5}$ &  54.8 $_{\pm0.2}$ &  55.1 $_{\pm0.4}$ &  56.2 $_{\pm0.2}$ &                 - &  52.5 $_{\pm0.0}$ &                 - &                 - &                 - &                 - &  47.0 $_{\pm0.5}$ &  54.3 $_{\pm0.0}$ &  54.2 $_{\pm0.3}$ &                 - &                 - &  55.4 $_{\pm0.1}$ &  55.0 $_{\pm0.5}$ &  54.4 $_{\pm0.2}$ &  53.2 $_{\pm0.3}$ \\
     & BPE &  52.7 $_{\pm0.5}$ &  54.5 $_{\pm0.3}$ &  45.1 $_{\pm0.4}$ &  55.5 $_{\pm0.2}$ &  55.9 $_{\pm0.2}$ &  58.7 $_{\pm0.2}$ &                 - &  53.0 $_{\pm0.2}$ &                 - &                 - &                 - &                 - &  44.5 $_{\pm0.1}$ &  53.8 $_{\pm0.5}$ &  55.5 $_{\pm0.2}$ &                 - &                 - &  57.2 $_{\pm0.2}$ &  55.2 $_{\pm0.6}$ &  54.5 $_{\pm0.2}$ &  53.5 $_{\pm0.3}$ \\
     & TokMix &  51.9 $_{\pm0.3}$ &  53.7 $_{\pm0.2}$ &  40.9 $_{\pm0.6}$ &  53.8 $_{\pm0.3}$ &  55.2 $_{\pm0.2}$ &  56.6 $_{\pm0.2}$ &                 - &  51.2 $_{\pm0.1}$ &                 - &                 - &                 - &                 - &  44.7 $_{\pm0.4}$ &  53.0 $_{\pm0.6}$ &  53.7 $_{\pm0.2}$ &                 - &                 - &  56.0 $_{\pm0.1}$ &  55.1 $_{\pm0.2}$ &  54.2 $_{\pm0.4}$ &  52.3 $_{\pm0.3}$ \\
\bottomrule
\end{tabular}
}
\caption{Results of evaluation for in language properties and tasks for twenty diverse languages.We observe significant changes for different tokenization methods.}
\label{tab:in_lang_table_20l}
% \end{adjustbox}
\end{table}
\end{landscape}
